First Experiences in Performance Benchmarking with the New SPEChpc 2021 Suites

Modern HPC systems are built with innovative system architectures and novel programming models to further push the speed limit of computing. The increased complexity poses challenges for performance portability and performance evaluation. The Standard Performance Evaluation Corporation -SPEC has a long history of producing industry standard benchmarks for modern computer systems. SPEC is a newly released SPEChpc 2021 benchmark suites, developed by the High Performance Group, are a bold attempt to provide a fair and objective benchmarking tool designed for state of the art HPC systems. With the support of multiple host and accelerator programming models, the suites are portable across both homogeneous and heterogeneous architectures. Different workloads are developed to fit system sizes ranging from a few compute nodes to a few hundred compute nodes. In this manuscript, we take a first glance at these benchmark suites and evaluate their portability and basic performance characteristics on various popular and emerging HPC architectures, including x86 CPU, NVIDIA GPU, and AMD GPU. This study provides a first-hand experience of executing the SPEChpc 2021 suites at scale on production HPC systems, discusses real-world use cases, and serves as an initial guideline for using the benchmark suites.

==> 06-discussion.tex <==
%Efforts in this paper highlight some of 
This work shows the rigorous testing conducted on four HPC clusters evaluating complex scientific applications implemented using MPI-only, MPI+ACC, and MPI+TGT programming models across four different workload sizes, that are at times compute- and otherwise memory-bound. 
%The experiments expose various flavors of the runs. 
The experiments and results expose various performance `flavors'.  
The experiments on large systems, such as Frontera, reveal how applications with small memory footprint achieve super-linear scaling. 
Other experiments on large clusters, such as those on Summit, showcase the need to even further increase the workload sizes of the applications in the \textit{large} suite to fully exploit Summit's scale.
Other observations include issues related to compiler/runtime components for accelerator offloading programming models. 
The best and the worst parallel efficiencies were observed on the state-of-the-art NVIDIA's A100 GPUs. 
Throughout the journey of building the SPEChpc~2021 benchmark suite, the authors also learnt about adjusting workload sizes starting from a few nodes and up to hundreds and thousands of nodes.

